Towards MAC/Anycast Diversity in IEEE 802.11n MIMO Networks

Opportunistic Routing (OR) is a novel routing technique for wireless mesh networks that exploits the broadcast nature of the wireless medium. OR combines frames from multiple receivers and therefore creates a form of Spatial Diversity, called MAC Diversity. The gain from OR is especially high in networks where the majority of links has a high packet loss probability. The updated IEEE 802.11n standard improves the physical layer with the ability to use multiple transmit and receive antennas, i.e. Multiple-Input and Multiple-Output (MIMO), and therefore already offers spatial diversity on the physical layer, i.e. called Physical Diversity, which improves the reliability of a wireless link by reducing its error rate. In this paper we quantify the gain from MAC diversity as utilized by OR in the presence of PHY diversity as provided by a MIMO system like 802.11n. We experimented with an IEEE 802.11n indoor testbed and analyzed the nature of packet losses. Our experiment results show negligible MAC diversity gains for both interference-prone 2.4 GHz and interference-free 5 GHz channels when using 802.11n. This is different to the observations made with single antenna systems based on 802.11b/g, as well as in initial studies with 802.11n.

==> outlook.tex <==
\section{Outlook}
tbd.

\tolja{Mögliche weiterfuerhende Forschung auf diesem Gebiet:
\begin{itemize}
  \item Was zeigen die Ergebnisse? Sollte der Standard bessere Signalfilter vorschreiben? Oder ist alles toll?
	\item 802.11n ACI model für einen Packetlevel Simulator wie NS3.
	\item Einfluss der Ergebnisse auf die Erforschung von Multi-channel MAC/NET Protokollen. Was bleibt noch? Ist das Thema noch aktuell? Wo sollte der Fokus liegen?
\end{itemize}
}

==> requirements.tex <==
\section{Requirements}\label{sec:requirements}
Tbd.
